Oolong: Evaluating Long Context Reasoning and Aggregation Capabilities

As model context lengths continue to grow, concerns about whether models effectively use the full context length have persisted. While several carefully designed long-context evaluations have recently been released, these evaluations tend to rely on retrieval from one or more sections of the context, which allows nearly all of the context tokens to be disregarded as noise. This represents only one type of task that might be performed with long context. We introduce Oolong, a benchmark of long-context reasoning tasks that require analyzing individual chunks of text on an atomic level, and then aggregating these analyses to answer distributional questions. Oolong is separated into two task sets: Oolong-synth, a set of naturalistic synthetic tasks, where we can easily ablate components of the reasoning problem; and Oolong-real, a downstream setting which requires reasoning over real-world conversational data. Oolong requires models to reason over large quantities of examples, to perform both classification and counting in-context, and to reason over temporal and user relations. Even frontier models struggle on Oolong, with GPT-5, Claude-Sonnet-4, and Gemini-2.5-Pro all achieving less than 50% accuracy on both splits at 128K. We release the data and evaluation harness for Oolong to enable further development of models that can reason over large quantities of text.

==> resources/plots/ablation_levels.tex <==
\begin{figure*}[h!]
    \centering
    \begin{subfigure}[]{0.55\textwidth}
        \input{resources/plots/synth_ablation_levels}
    \end{subfigure}
    \hfill
    \begin{subfigure}[]{0.35\textwidth}
        \input{resources/plots/real_ablation_levels}
    \end{subfigure}
    \caption{Comparison across reasoning levels.}
    \label{fig:ablation_reasoning_levels}
\end{figure*}

==> resources/plots/ablations_short_and_labels.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[]{0.4\textwidth}
        \input{resources/plots/synth_ablation_labels}
    \end{subfigure}
    \hfill
    \begin{subfigure}[]{0.5\textwidth}
        \input{resources/plots/synth_analysis_short_context}
    \end{subfigure}
    \caption{Comparison on \ours-synth: (a) we provide the gold labels in the input. This leads to a consistent but small improvement, (b) short context performance; while the top models have similar short-context performance, differences emerge as the context length grows.}
    \label{fig:ablation_short_and_labels}
\end{figure*}

==> resources/tables/oolong_real_sample.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{p{0.97\textwidth}}
\toprule
\emph{Counting} \\
\midrule
Total number of rolls in this episode? \\
What is the count of Crits? (natural rolls of value 1 or 20)? \\
How many \{spell type\} spells were cast during this episode? \\
How many characters cast \{spell name\} spell all across episodes? \\
What is the second spell cast in the episode \{episode index\}? \\
\midrule
\emph{Enumeration} \\
\midrule
What are the first \{count\} spells cast in this episode? Return a comma separated list. \\
List the last spell cast in each episode? Return a comma separated list. \\
\midrule
\emph{Indexing} \\
\midrule
What is the cumulative total of rolls by the end of episode \{episode index\}? Count the
number of rolls and not the values of the rolls. \\
What is the second spell cast in the episode \{episode index\}? \\
List the last spell cast in each episode? Return a comma separated list. \\
\bottomrule
\end{tabular}
\caption{Question types covered in \ours-real dataset.}
\label{tab:oolong_real_sample}
\end{table*}

==> resources/tables/oolong_synth_by_task.tex <==
\begin{table*}[t]
\begin{tabular}{@{}llll@{}}
\toprule
Model              & Counting tasks & User tasks & Timeline tasks \\ \midrule
Random baseline    &                &            &                \\
Claude 4 Sonnet    &                &            &                \\
Gemini 2.5 Flash   &                &            &                \\
Deepseek R1 -- May &                &            &                \\
Llama 4 Maverick   &                &            &                \\
Grok 4             &                &            &                \\
GPT 5              &                &            &                \\
GPT 4.1-mini       &                &            &                \\
GPT o4-mini        &                &            &                \\ \bottomrule
\end{tabular}
\end{table*}

==> resources/tables/reasoning_trace_analysis.tex <==
\begin{table*}[t]
\begin{tabular}{lll}
\hline
Behavior                                                           & Claude Sonnet 4 & Deepseek R1 0528 \\ \hline
Labeling at least one instance from the input                      &                 &                  \\
Copying sections of the input (e.g. enumerating relevant examples) &                 &                  \\
Describing the problem as too hard, intractable, or impossible     &                 &                  \\
Debating whether or not to label each example                      &                 &                  \\ \hline
\end{tabular}
\caption{Common reasoning trace patterns from the two reasoning models with visible thinking. \amanda{todo: add more info}}
\label{tab:reasoning_behaviors}
\end{table*}
